DyCAF-Net: Dynamic Class-Aware Fusion Network

Recent advancements in object detection rely on modular architectures with multi-scale fusion and attention mechanisms. However, static fusion heuristics and class-agnostic attention limit performance in dynamic scenes with occlusions, clutter, and class imbalance. We introduce Dynamic Class-Aware Fusion Network (DyCAF-Net) that addresses these challenges through three innovations: (1) an input-conditioned equilibrium-based neck that iteratively refines multi-scale features via implicit fixed-point modeling, (2) a dual dynamic attention mechanism that adaptively recalibrates channel and spatial responses using input- and class-dependent cues, and (3) class-aware feature adaptation that modulates features to prioritize discriminative regions for rare classes. Through comprehensive ablation studies with YOLOv8 and related architectures, alongside benchmarking against nine state-of-the-art baselines, DyCAF-Net achieves significant improvements in precision, mAP@50, and mAP@50-95 across 13 diverse benchmarks, including occlusion-heavy and long-tailed datasets. The framework maintains computational efficiency ($\sim$11.1M parameters) and competitive inference speeds, while its adaptability to scale variance, semantic overlaps, and class imbalance positions it as a robust solution for real-world detection tasks in medical imaging, surveillance, and autonomous systems.

==> sec/0_abstract.tex <==
\begin{abstract}
Recent advancements in object detection rely on modular architectures with multi-scale fusion and attention mechanisms. However, static fusion heuristics and class-agnostic attention limit performance in dynamic scenes with occlusions, clutter, and class imbalance. We introduce \ul{Dy}namic \ul{C}lass-\ul{A}ware \ul{F}usion \ul{Net}work (DyCAF-Net) that addresses these challenges through three innovations: (1) an input-conditioned equilibrium-based neck that iteratively refines multi-scale features via implicit fixed-point modeling, (2) a dual dynamic attention mechanism that adaptively recalibrates channel and spatial responses using input- and class-dependent cues, and (3) class-aware feature adaptation that modulates features to prioritize discriminative regions for rare classes. Evaluated on 13 benchmarks, DyCAF-Net achieves state-of-the-art results, improving mAP@50–95 by 9.91\% on Axial MRI (imbalance ratio: 5.54) and 3.38\% on Mask Wearing (occlusion-heavy), with precision gains of 25.70\% and 7.82\%, respectively. While recall occasionally dips (e.g., –23.51\% on Axial MRI), DyCAF-Net achieves higher mAP@50–95 in 10/13 datasets, outperforming graph-based (e.g., +25.7\% mAP@50–95 over TGAT) and temporal models. Critically, DyCAF-Net exhibits consistent net average improvements over the next best-performing model across all datasets: +1.56\% in Precision, +1.56\% in mAP@50, and +2.45\% in mAP@50–95. The framework maintains parameter efficiency ($\sim$11.1M parameters) and competitive inference speeds ($\simeq$14.66\,ms), validating its robustness to scale heterogeneity, semantic overlaps, and imbalance. The code of DyCAF-Net is available at \url{https://github.com/Abrar2652/DyCAF-NET}.
\end{abstract}


.




